Debiasing Made State-of-the-art: Revisiting the Simple Seed-based Weak Supervision for Text Classification

Recent advances in weakly supervised text classification mostly focus on designing sophisticated methods to turn high-level human heuristics into quality pseudo-labels. In this paper, we revisit the seed matching-based method, which is arguably the simplest way to generate pseudo-labels, and show that its power was greatly underestimated. We show that the limited performance of seed matching is largely due to the label bias injected by the simple seed-match rule, which prevents the classifier from learning reliable confidence for selecting high-quality pseudo-labels. Interestingly, simply deleting the seed words present in the matched input texts can mitigate the label bias and help learn better confidence. Subsequently, the performance achieved by seed matching can be improved significantly, making it on par with or even better than the state-of-the-art. Furthermore, to handle the case when the seed words are not made known, we propose to simply delete the word tokens in the input text randomly with a high deletion ratio. Remarkably, seed matching equipped with this random deletion method can often achieve even better performance than that with seed deletion.

==> files/3-prelims.tex <==
\section{Problem and Motivation}
% \chengyu{We consider the confidence learning only. So the experiments here should show random noise greatly improves confidence learning}
    % \item \sout{self-training performance. Controlled experiments between feature-dependent and feature-independent label noise show that feature-independent label noise is even better than optimal selection (correct only)} % this is not confidence learning
    
    % \item Other problems (e.g. backdoor) caused by feature-dependent label nois


\smallsection{Label bias in weak supervision ruins confidence learning} % Label bias (feature-dependent label noise)
% \todo{Delete this}
% However, the confidence score may not be meaningful, in particular, for selecting pseudo-labels in weak supervision. This is because weak supervision often consists of one or a set of rules, which may inject erroneous but simple correlations between the pseudo-labels and the input sequence. Upon training, a classifier can easily learn such rules, thus yielding high confidence on any inputs that match such rules. Subsequently, the learned uncertainty may not be a useful measure of the probability of label error at all. 

\todo{Move to caption in Figure 1}
In Figure~\ref{figure:noise-coverage}, we train a classifier on all the pseudo-labels and select a subset of the pseudo-labels based on its confidence score. We found that the noise rate in the selected pseudo-labels is high regardless of the selection ratio. On some datasets such as 20News-Fine, the noise rate is almost constant as we vary the selection ratio, which implies that the confidence score may be completely random values.  
% \todo{In Figure~\ref{}}, we further train (or self-train) a classifier on the selected pseudo-labels and found that the performance is no better, and often significantly worse, than training on all pseudo-labels.

% \chengyu{mention a little bit of theory, feature-dependency of label bias}



\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/noise-transition-matrix.pdf}
    \vspace{-6mm}
    \caption{Noise transition matrix 
    }
    \label{figure:noise-transition-matrix}
\end{figure}

\smallsection{Feature-independent label noise will not hurt confidence learning}
% \todo{Move to appendix, leave a pointer in the intro}
\todo{Move to caption} 
Interestingly, we found that a model trained on feature-independent label noise, typically referred to as random flipping label noise, largely does not affect learning proper confidence. To demonstrate this, we synthesize feature-independent label noise to allow fair comparison with the label noise introduced by weak supervision. Specifically, we randomly select a pseudo-label for each document in the same pseudo-labeled dataset, while ensuring the overall noise rate, noise rate in each class, and the noise transition rate between any two classes are identical to the label noise induced by weak supervision. Figure~\ref{figure:noise-transition-matrix} confirms the noise transition matrix of the synthesized feature-independent label noise is indeed the same as that of weak supervision. 

However, drastically different from the feature-dependent label noise, Figure~\ref{figure:noise-coverage} shows the confidence score of a classifier trained on such label noise can in fact genuinely reflect the probability of error of a given pseudo-label. 
% \chengyu{but in terms the pseudo-labels of weak supervision or labels in this synthetic case?}\chengyu{Should be the former}. 
% Subsequently, the classifier trained on the subset of pseudo-labels selected based on such confidence can also achieve much higher classification performance. \maybe{todo}.

    
% \smallsection{Theoretical analysis of uncertainty learning on feature-independent label noise}
% \maybe{Theory}
    


% \chengyu{Try perform random deletion in all self-training iterations except the last one? Will this help the performance even more, especially for fine-grained datasets?}


